Resolving Stellar Populations outside the Local Group: MAD observations of UKS2323-326

We present a study aimed at deriving constraints on star formation at intermediate ages from the evolved stellar populations in the dwarf irregular galaxy UKS2323-326. These observations were also intended to demonstrate the scientific capabilities of the multi-conjugated adaptive optics demonstrator (MAD) implemented at the ESO Very Large Telescope as a test-bench of adaptive optics (AO) techniques. We perform accurate, deep photometry of the field using J and Ks band AO images of the central region of the galaxy. The near-infrared (IR) colour-magnitude diagrams clearly show the sequences of asymptotic giant branch (AGB) stars, red supergiants, and red giant branch (RGB) stars down to ~1 mag below the RGB tip. Optical-near-IR diagrams, obtained by combining our data with Hubble Space Telescope observations, provide the best separation of stars in the various evolutionary stages. The counts of AGB stars brighter than the RGB tip allow us to estimate the star formation at intermediate ages. Assuming a Salpeter initial mass function, we find that the star formation episode at intermediate ages produced ~6x10^5 M_sun of stars in the observed region.

==> uksDefs.tex <==
\newcommand{\uks}{UKS\,2323-326}
\newcommand{\mh}{{\rm [M/H]}}
\newcommand{\feh}{{\rm [Fe/H]}}

\newcommand{\ebv}{\mbox{$E_{B\!-\!V}$}}

\newcommand{\marco}[1]{{\color{red}\textbf {#1}}}
%\newcommand{\evh}[1]{{\color{blue}\textbf {#1}}}
\newcommand{\evh}[1]{{#1}}

\newcommand{\referee}[1]{{\textbf {#1}}}
%\newcommand{\referee}[1]{{#1}}

